Deep Diffeomorphic Normalizing Flows

The Normalizing Flow (NF) models a general probability density by estimating an invertible transformation applied on samples drawn from a known distribution. We introduce a new type of NF, called Deep Diffeomorphic Normalizing Flow (DDNF). A diffeomorphic flow is an invertible function where both the function and its inverse are smooth. We construct the flow using an ordinary differential equation (ODE) governed by a time-varying smooth vector field. We use a neural network to parametrize the smooth vector field and a recursive neural network (RNN) for approximating the solution of the ODE. Each cell in the RNN is a residual network implementing one Euler integration step. The architecture of our flow enables efficient likelihood evaluation, straightforward flow inversion, and results in highly flexible density estimation. An end-to-end trained DDNF achieves competitive results with state-of-the-art methods on a suite of density estimation and variational inference tasks. Finally, our method brings concepts from Riemannian geometry that, we believe, can open a new research direction for neural density estimation.

==> experiments.tex <==
% !TEX root = ../submission-v3.tex
\section{Experimental Results}

\subsection{Approximation of an ODE-Solver}\label{sec:ode_approx}
As we discussed in section~\ref{sec:vel_stat}, our proposed flow is basically approximating an ODE solver by integrating a constant velocity vector field over time. For traditional ODE-solvers, as the time step gets smaller, the accuracy of the solver improves. In our architecture, this phenomena is equivalent to having more RNN blocks and therefore smaller integration step $\Delta t$. 

Figure~\ref{fig:ode_solver} shows the L2 error between in the solution given by an ODE-solver and the solution of the RNN flow for integrating a constant velocity field over time. The plot shows how the accuracy of our model in approximating an ODE solver increases as the number of RNN blocks increase. In practice, we found that a flow of 8 RNN blocks works pretty well, and this corresponds to the knee point that can be seen in the plot of Figure~\ref{fig:ode_solver}.

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/ode_approx.PNG}
    \caption{The L2 error between an ODE-solver solution and our RNN flow solution of integrating a constant velocity field over time.}
    \label{fig:ode_solver}
\end{figure}

\subsection{Inversion Quality}
In this section, we present empirical results that shows how the quality of the inversion of our flow can be controlled by varying the number of RNN cells in this flow. Figure~\ref{fig:inversion_quality} shows the L2 distance error between the a bunch of random points that are passed forward and their corresponding inverted samples that are passed backward through the flow. The plot shows how the inversion error decreases as the number of RNN blocks composing the flow increases. This ties back to similar reasons why the more blocks leads to better approximation of the ODE solver (as presented in section~\ref{sec:ode_approx} because the inversion flow is essentially integrating the negative of the constant velocity vector field that constitutes the forward flow. Therefore, increasing the number of RNN blocks is equivalent to decreasing the integration step $\Delta t$ which leads to more accurate inversion.

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/inversion_quality.PNG}
    \caption{The average L2 error between random samples passing through the RNN flow and their corresponding inverted samples resulting from the backward pass through the RNN flow. The error is averaged over 50 experiments each with 1000 random samples passed through the flow.}
    \label{fig:inversion_quality}
\end{figure}

\subsection{Regularization Effect}
In this section, we show experiments that reflect the effect of the Regularization techniques discussed in Section.~\ref{sec:regularizing_the_flow}.
\paragraph{Velocity Shrinkage:}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/regularization_effect.PNG}
    \caption{The effect of regularizing our flow. For small number of cells, training tends to be unstable as the KL-divergence diverge. Regularizing the model using the norm of the integral of the velocity field over time tends to stabilize training and lead better results of the distribution estimation.}
    \label{fig:regularization_effect}
\end{figure}

\subsection{Approximating Complex Distributions}
In this section, we show the performance of our proposed flow on the task of sampling from a given distribution,

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/density_regeneration_3.PNG}
    \caption{(a) The ground truth distribution to sample from. (b) The sampled distributions using our flow. (c) The sampled distribution using the NF \citep{rezende2015variational}. (c) The sampled distribution using NAF \citep{huang2018neural}}
    \label{fig:distribution_regeneration}
\end{figure}


\subsection{Skewed Posterior}
\begin{figure*}[t]
    \centering
    \includegraphics[width=.8\linewidth]{figures/skewed_posterior.pdf}
    \caption{}
    \label{fig:skewed_posterior}
\end{figure*}

\subsection{Variational Auto-encoder}

\subsubsection{MNIST}
\begin{table}[t]
\centering
\caption{Comparison of the elbo on the test set for the  MNIST dataset. The reported results are averaged over three experiments.}
\label{table:MNIST_comparisons}
\small
\begin{tabular}{l|c}
Model  &  -ELBO\\ \hline \hline
Vanilla VAE (diagonal covariance) & 151.9\\
VAE-NF \citep{rezende2015variational} &  150.6 \\
RNN Flow - ours &  149.7 \\
VAE-NAF \citep{huang2018neural} & 147.5 \\
\hline
\end{tabular}
\end{table}

\subsubsection{CIFAR-10}

% \subsubsection*{Acknowledgments}



